Beginner's Lecture Notes on Quantum Spin Chains, Exact Diagonalization and Tensor Networks

Aimed at introducing readers to the physics of strongly correlated many-body systems, these notes focus on numerical methods, with detailed discussions on implementing working code for exact diagonalization. A brief introduction to tensor network methods is also included. Prepared for the Summer School Quantumandu, held at Tribhuvan University (Kathmandu, Nepal) from 25 to 31 July 2024, as part of the ICTP's Physics Without Frontiers program, these notes are primarily intended for readers encountering this field for the first time.

==> Lectures/Lecture_phase_transition_1.tex <==
\chapter{Classical Phase Transitions}\label{ch:cpt}

\section{Phenomenology}

\begin{figure}\label{fig:magnetic_domain}
    \centering
\includegraphics[width=0.75\linewidth]{Pictures/magnetic_domain.pdf}
\caption{Ordered and disordered phases of a ferromagnetic system.}
\end{figure}

Atoms in certain materials possess an intrinsic magnetic dipole moment, arising from the spin and orbital motion of their electrons. In most materials, however, these magnetic dipoles are randomly oriented, causing them to cancel each other out and resulting in no net magnetic field.

However, in some materials, such as iron or cobalt, interactions between atomic dipoles create a noticeable overall magnetic field. This occurs in \textit{ferromagnetic materials} when the temperature is below a specific critical value called the Curie temperature ($T_{c}$), which varies by material. At Curie temperature, these materials undergo a \textit{phase transition}, changing their physical properties. In this case, the change is the spontaneous alignment of microscopic dipoles, resulting in a macroscopic magnetic field. This phase transition occurs due to two competing factors. 

\begin{itemize}
\item \textbf{Energy Minimization} --
In ferromagnetic materials, the magnetic dipoles (or spins) of each atom tend to align to minimize the system's total energy. This alignment occurs due to quantum effects, but it can also be modelled classicaly. If energy minimization were the sole governing principle, all these dipoles (spins) would align perfectly, causing many materials to exhibit a strong magnetic field. However, this is not observed in practice because a competing mechanism—thermal fluctuations—comes into play, disrupting perfect alignment.

\item \textbf{Entropy Maximisation} --
Among the many possible configurations of a system, those where spins align in the same direction are rare. Unless it requires a lot of energy to reorient neighboring spins, there are far more configurations with randomly oriented spins than with fully aligned spins. Entropy $S $, which measures disorder, is given by Boltzmann's formula:
\begin{equation}\label{eq:entropy}
    S(E) = k \log \omega(E)
\end{equation}
where $\omega(E)$is the number of states at energy $E $, and $k$is the Boltzmann constant. If systems only sought to maximize disorder, spontaneous magnetization would never occur.

\end{itemize}
As illustrated by the example of magnetic dipoles, macroscopic physical systems with a vast number of degrees of freedom are influenced by two competing tendencies: one that seeks to order the system to minimize energy, and another that promotes disorder to maximize entropy. or a genuine competition between these tendencies, an additional critical factor must be considered: the system's temperature. The role of temperature $T$in this context is specified by the principles of statistical mechanics.

\subsection{Classification of the phase transitions}
In modern physics, phase transitions are classified into two main types: first-order and second-order phase transitions.

\begin{itemize}
    \item \textbf{First-order phase transitions} involve a latent heat. This means that at the transition point, the system absorbs or releases a fixed amount of energy while the temperature remains constant. These transitions are marked by a finite correlation length, leading to a mixed-phase state where parts of the system have completed the transition while others have not. For example, when water cools to its freezing point $T_f $, it doesn't instantly turn to ice but instead forms a mixture of water and ice. The latent heat indicates a significant structural change in the material: above $T_f $, water molecules move freely in a disordered manner, while below $T_f $, they are arranged in an orderly crystal lattice of ice. Other examples of first-order transitions include Bose–Einstein condensation.
    \item \textbf{Second-order phase transitions}, also known as continuous phase transitions, do not involve latent heat. Instead, they are characterized by a divergence of the correlation length at the critical point. Examples include the ferromagnetic transition, superconductors, and the superfluid transition. Landau developed the first phenomenological theory of these transitions. 
\end{itemize}

There are also ``infinite-order phase transitions'', which are continuous but do not break any symmetries. A well-known example is the Kosterlitz–Thouless transition in the two-dimensional XY model. 

\section{Brief review of Statistical Physics}
One of the most significant advancements in nineteenth-century physics was the discovery of the understanding of the statistical laws governing many-body systems at thermal equilibrium. These laws form the foundation of statistical mechanics and have become a cornerstone of modern theoretical physics.

Let $\pmb{\sigma}$ represent a generic state (configuration) of a physical system, such as the orientation of each magnetic dipole. For a system at thermal equilibrium with a large number $N$ of spins / particles, the probability $p(\pmb{\sigma})$ of observing the system in a given configuration $\pmb{\sigma}$ is given by the Boltzmann law
\begin{equation}
    p(\pmb{\sigma}) = \frac{e^{-\beta H(\pmb{\sigma})}}{Z} \, ,
\end{equation}
where $H(\pmb{\sigma})$ is the energy of the configuration $\pmb{\sigma}$, $\beta = \frac{1}{kT}$ with $k$ being the Boltzmann constant, and $T$ the absolute temperature. The partition function $Z$ is defined as
\begin{equation}
Z = \sum_{\pmb{\sigma}} e^{-\beta H(\pmb{\sigma})} \, ,
\end{equation}
and normalizes the Boltzmann probabilities, also encoding all relevant physical information about the system at equilibrium. If we rewrite this sum by grouping together all configurations $\pmb{\sigma}$ that share the same energy $E = H(\pmb{\sigma})$, we obtain:
\begin{equation}
Z = \sum_{E} \omega(E) e^{-\beta E} \, ,
\end{equation}
where $\omega(E)$ is the total number of configuration with energy $E$. Now, by using the definition of entropy (Eq.\ref{eq:entropy}), we get
\begin{equation}
Z = \sum_{E}  e^{-\beta E + \log \omega(E)}
= \sum_{E}  e^{-\beta \left(E - T S(E) \right)} \, .
\end{equation}
The \textit{free energy} $F$ is related to $Z$ by:
\begin{equation}
Z \equiv e^{-\beta F(N, \beta)} \, ,
\end{equation}
where $F$ is given by:
\begin{equation}
F = U - TS \, .
\end{equation}
Here, $U = \langle E \rangle$ is the internal energy, and $S$ is the entropy. The thermodynamic relations for $U$ and $S$ are:
\begin{equation}
\langle U \rangle = \frac{\partial (\beta F)}{\partial \beta}
, \quad
\langle S \rangle = \beta^2 \frac{\partial F}{\partial \beta} \, .
\end{equation}
These equations highlight how the balance between energy and entropy changes with temperature, potentially leading to phase transitions at a critical temperature $T_c$.

\section{The Peierls argument}

The Peierls argument provides a way to understand phase transitions by considering the stability of ordered states against the formation of domain walls. Domain walls are boundaries separating regions with different spin orientations. If creating these walls costs too much energy, the system prefers to remain ordered, leading to a phase transition at a certain temperature.

\subsubsection{The Ising Model in 1D}

In the 1D Ising model, we have spins $\spin_i = \pm 1$ on a line, with the Hamiltonian $H = -J \sum_{i} \spin_i \spin_{i+1}$, where $J > 0$is the coupling constant.

\begin{enumerate}
    \item \underline{Domain Wall Energy}: 
    \begin{itemize}
        \item In 1D, a domain wall is a boundary between two spins pointing in opposite directions.
        \item The energy cost to create one domain wall is $2J$because it breaks two bonds.
    \end{itemize}
    
    \item \underline{Entropy Consideration}: 
    \begin{itemize}
        \item The number of possible positions for a domain wall in a system with $N$spins is $N $.
        \item The entropy associated with placing a domain wall is $k_B \ln(N) $.
    \end{itemize}
    
    \item \underline{Free Energy}: 
    \begin{equation}
    \Delta F = 2J - k_B T \ln(N).
    \end{equation}
\end{enumerate}

At any finite temperature $T $, the entropy term $k_B T \ln(N)$will eventually dominate for large $N $, making $\Delta F$negative. This implies that creating domain walls becomes favorable, leading to a disordered phase. Therefore, no long-range order (ferromagnetic order) is expected at any finite temperature in the 1D Ising model.

\subsubsection{The Ising Model in 1D}

In the 2D Ising model, spins are arranged on a lattice, and the Hamiltonian is $H = -J \sum_{\langle i,j \rangle} \spin_i \spin_j$, 
where the sum runs over nearest neighbor spins.

\begin{enumerate}
    \item \underline{Domain Wall Energy}: 
    \begin{itemize}
        \item In 2D, a domain wall is a line of flipped spins separating regions with different orientations.
        \item The energy cost of a domain wall is proportional to its length $L $, so $\Delta E \approx 2JL $.
    \end{itemize}
    
    \item \underline{Entropy Consideration}: 
    \begin{itemize}
        \item The number of ways to arrange a domain wall of length $L$ is exponential in $L$, $\exp(L)$.
        \item The entropy associated with a domain wall of length $L$ is $k_B L \ln 2 $.
    \end{itemize}
    
    \item \underline{Free Energy}: 
    \begin{equation}
    \Delta F = 2JL - k_B T L \ln 2.
    \end{equation}
\end{enumerate}

At low temperatures, the energy term $2JL$ dominates, making $\Delta F$ positive, and domain walls are not favorable. This leads to long-range order and a finite temperature transition in the 2D Ising model. However, as the temperature increases, the entropy term $k_B T L \ln 2$ starts to dominate, and $\Delta F$ can become negative, favoring domain wall creation and leading to a disordered phase. This transition occurs at a critical temperature $T_c$.

We can estimate the critical temperature $T_c$ for the 2D Ising model by equating the energy and entropy contributions:
\begin{equation}
2JL \approx k_B T_c L \ln 2 
\end{equation}
which gives $T_c \approx \frac{2J}{k_B \ln 2}$. While this is a rough estimation, it captures the idea that a phase transition occurs when the thermal energy is comparable to the energy cost of creating domain walls.

\section{Exact solution of the Ising model in 1D}
The partition function of the 1D Ising model can be computed exactly using the transfer matrix approach. This method is a powerful tool to solve statistical mechanics problems, particularly in one dimension.

We consider a 1D Ising Hamiltonian 
\begin{equation}
H(\pmb{\sigma}) = -J \sum_{i=1}^N \spin_i \spin_{i+1} - h \sum_{i=1}^{N} \spin_i \, ,
\end{equation}
where $J$ is the coupling constant and $h$ is the external magnetic field. For simplicity, we assume periodic boundary conditions: $\spin_{N+1} = \spin_1$. The partition function $Z$ is given by:
\begin{equation}
Z = \sum_{\pmb{\sigma}} \exp\left(-\beta H\right)
\end{equation}
where $\beta = \frac{1}{k_B T}$, $k_B$ is the Boltzmann constant, and $T$ is the temperature. Now, we rewrite the Hamiltonian in terms of a certain $2 \times 2$ matrix $\mathcal{T}$ named \textit{transfer matrix}. The transfer matrix elements are defined as:
\begin{equation}
\mathcal{T}(\sigma_i, \sigma_{i+1}) = \exp\left[ \beta (J \sigma_i \sigma_{i+1} + \frac{h}{2}(\sigma_i + \sigma_{i+1})) \right]
\end{equation}
thus the matrix reads
\begin{equation}
\mathcal{T} = \begin{pmatrix}
\exp(\beta J + \beta h) & \exp(-\beta J) \\
\exp(-\beta J) & \exp(\beta J - \beta h)
\end{pmatrix}
\end{equation}

The partition function $Z$ is then given by:
\[
Z = \text{Tr}(\mathcal{T}^N)
\]

To compute $\mathcal{T}^N$, we first diagonalize $\mathcal{T}$. Let $\lambda_1$ and $\lambda_2$ be the eigenvalues of $\mathcal{T}$. The eigenvalues are found by solving the characteristic equation:
\[
\det(\mathcal{T} - \lambda I) = 0
\]

The eigenvalues $\lambda_1$ and $\lambda_2$ are:
\begin{equation}
\lambda_{1,2} = \exp(\beta J) \cosh(\beta h) \pm \sqrt{\exp(2 \beta J) \sinh^2(\beta h) + \exp(-2 \beta J)} \, .
\end{equation}
Then $\mathcal{T}^N$ can be written as:
\[
\mathcal{T}^N = M \begin{pmatrix}
\lambda_1^N & 0 \\
0 & \lambda_2^N
\end{pmatrix} M^{-1}
\]
where $P$ is the matrix of eigenvectors.

Thus, the partition function is:
\begin{equation}
Z = \lambda_1^N + \lambda_2^N \,.
\end{equation}
For large $N$, the largest eigenvalue $\lambda_1$ dominates:
\begin{equation}
Z \approx \lambda_1^N \, .
\end{equation}
In one dimension, the largest eigenvalue $\lambda_1$ always dominates the partition function for any finite temperature. As a result, the free energy 
\begin{equation}
    F = -k_B T \ln Z \approx - N k_B T \log \lambda_1
\end{equation}
is an analytical function of the temperature $T$, for all $T>0$. This analyticity implies that there is no phase transition at any finite temperature. Thus, the analytical findings using the transfer matrix approach corroborate what is predicted by the Peierls argument regarding the absence of a phase transition in 1D.



